DEPAS: A Decentralized Probabilistic Algorithm for Auto-Scaling

The dynamic provisioning of virtualized resources offered by cloud computing infrastructures allows applications deployed in a cloud environment to automatically increase and decrease the amount of used resources. This capability is called auto-scaling and its main purpose is to automatically adjust the scale of the system that is running the application to satisfy the varying workload with minimum resource utilization. The need for auto-scaling is particularly important during workload peaks, in which applications may need to scale up to extremely large-scale systems. Both the research community and the main cloud providers have already developed auto-scaling solutions. However, most research solutions are centralized and not suitable for managing large-scale systems, moreover cloud providers' solutions are bound to the limitations of a specific provider in terms of resource prices, availability, reliability, and connectivity. In this paper we propose DEPAS, a decentralized probabilistic auto-scaling algorithm integrated into a P2P architecture that is cloud provider independent, thus allowing the auto-scaling of services over multiple cloud infrastructures at the same time. Our simulations, which are based on real service traces, show that our approach is capable of: (i) keeping the overall utilization of all the instantiated cloud resources in a target range, (ii) maintaining service response times close to the ones obtained using optimal centralized auto-scaling approaches.

==> 3-context.tex <==
\section{Context and Problem}
\label{sec:context}

Nowadays the area of cloud computing is giving to the research community important challenges to solve classical issues in cloud applications. These challenges regard functional aspects, including cloud toolkits and how to exploit them to build cloud applications, and non-functional aspects, including the possibility to take advantage of innovative cloud capabilities to increase the quality of the cloud applications and reduce their costs. The most important challenge comes from the fact that some cloud computing toolkits such as~\cite{leadsopennebula,nimbusproject,nurmi2009eucalyptus} are being extended to support auto-scaling, load-balancing, and multi-cloud capabilities. These functionalities allow a rational use of cloud resources, where a resource, depending on the considered cloud infrastructure, is a container for running applications, such as virtual machines or generic application servers. Auto-scaling gives to cloud applications the capability to request and release resources from the cloud infrastructure to meet the service demand of its users and avoid underutilization and overutilization. Load-balancing allows cloud applications to diffuse the application load to all the resources that have been allocated in the cloud infrastructure. Multi-cloud capabilities are offered by such systems (called multi-cloud or \emph{Sky} computing systems~\cite{keahey2009sky}) that may allocate resources in different clouds.

The existing cloud computing toolkits cited above already offer an abstraction to implement the capability of having different underlying clouds, and auto-scaling/load-balancing over time. However the solutions offered are centralized or hierarchical, meaning that the decisions to perform auto-scaling and load-balancing actions are made by a centralized controller that is typically offered by the cloud provider. These solutions are well known and used, but may become inadequate in contexts in which the cloud has unreliable nodes, for examples in scenarios in which the cloud resources are offered by small companies or even home users that want to share some unused computational power. In this kind of scenarios an application may experience a continuous unpredictable loss of resources, or, because of Internet connectivity problems, it may also have a consistent instantaneous loss of resources. %Finally in this kind of scenario the cloud cannot be designed to be centralized or under single ownership, therefore multi-cloud capabilities would be heavily exploited.

In the rest of this section we define the context in which our work is supposed to be used and a statement of the problem we want to solve.

\subsection{Context}
\label{sub:context}

The context we are considering is a generic cloud system that offers resources able to host batch services. The characteristics of these batch services is that all the data needed to be processed is given as input, and they return the result when the processing is completed. Compared to a generic service there is no interaction within the same service invocation and the resource that runs the service does not keep the state of the service between invocations. If a state needs to be maintained, then such state is written in a storage utility that is external to the resource (for example a NFS-like distributed storage). Examples of this kind of services are multimedia file conversions (audio and video file transcoding), scientific processing (such as the ones performed on volunteer computing infrastructures, such as SETI@Home), strong encryption/decryption, distributed compilation, translation, finding good solutions for NP-hard problems from a model, and any other kind of use in which some input data needs to be transformed in output data in a fast way. There are already services on the Internet that offer this kind of services to the general public such as~\cite{zencoder,ankoder} for the video file transcoding. In this context the functional requirements are not usually a problem since besides licensing issues, every public or privately owned platform is able to offer these services. The real issue is the cost for instantiating these services and the satisfaction of the customers that are willing to pay for using them. 

\begin{figure}
    \begin{center}
        \includegraphics[scale=0.4]{images/cloudinfrastructure.png}
        \caption{Cloud Infrastructure}
        \label{fig:cloudinfrastructure}
    \end{center}
\end{figure}

A typical cloud infrastructure is composed of the following entities (see Figure~\ref{fig:cloudinfrastructure}):
\begin{itemize}
\item \emph{Cloud infrastructure}: is the cloud itself as it is seen from the external world, an example is Amazon EC2~\cite{ec2}. It is composed of a controller and several physical machines.
\item \emph{Cloud controller}: it is a special physical machine (or a set of physical machines, depending on the implementation) that offers the possibility to instantiate and release resources through some API available to customers and an interaction with physical machine hypervisors.
\item \emph{Physical machine}: it is a piece of hardware that is able to host (virtualized) resources and a hypervisor for managing them. 
\item \emph{Hypervisor}: it is a software that creates, monitors, and destroys the resources of a physical machine.
\item \emph{Resources}: they are the computational resources actually instantiated in the physical machine. Depending on the implementation they can be Virtual Machines (VMs) or application servers. The purpose is to actually execute individual services or applications. 
\end{itemize}

Observing the current implementation of cloud applications we can see that one significant source of cost is the infrastructure's cost, which may be the cost (financial and environmental) for owning a private cloud infrastructure or for renting the resources from an external cloud infrastructure. Such costs are not only financial, but also environmental due to the energy consumption needed to keep the physical machines running. Another source of cost is the maintenance required to correctly provision the architecture to avoid having under or overutilized resources. To reduce these costs we need a mechanism to automatically allocate the resources (auto-scaling), redistribute the load (load-balancing), and deciding which kind of resource to allocate when they can have different characteristics (different allocation costs or different capacities). Actually, in infrastructures like EC2~\cite{ec2}, we have a decision-making component to perform the tasks above on top of the Cloud Controller and Hypervisor, meaning that it is conceptually centralized, but in a generic cloud infrastructure that may not be the only option. In fact it is also possible to make the decisions in an alternative and decentralized way in the form of a distributed specialized component, called \emph{Autonomic Manager}, that runs inside the resource with the actual service. 
%We will see in the next subsection how the introduction of an autonomic manager component inside the resource can help to achieve the goals of the approach we will present in the rest of this paper.

\subsection{Problem}
\label{sub:problem}

Under the generic context described in the previous section our goal is to define a generic architecture and a collection of algorithms to support the deployment and the provisioning of generic services in a cloud system. In particular we want to provide a solution that is able to work in an efficient way also in perturbed systems in which the resources are heterogenous in terms of \emph{computational capacity}, defined as the number of operations that a resource is able to execute in a time unit. Beside this we want also a solution that works in situations in which we have more than one cloud infrastructure, and in which there may be thousands of cheap and unreliable resources that cannot share the full knowledge of all the other resources of the system. It is widely known from the P2P area~\cite{milojicic2002peer} that using a classical centralized/hierarchical approach in a high-scale system in which nodes are unreliable and with local knowledge only may produce high management and coordination costs. These costs are due to the rebuilding of the structure of the system in case of failure of the central points. Another problem is that a multi-cloud system should be neutral with respect to individual cloud infrastructures, therefore monitoring and allocation decisions should be taken at the resource level (the only ones directly controlled by the service provider) instead of having a centralized global network of supervisors built on top of components owned by the cloud provider (such as hypervisors or cloud controllers, as typically found in current commercial solutions such as~\cite{auto-scaling}).

%In conclusion the main actor will be an autonomic manager component that will run at the 
To obtain a level of transparency with respect to each individual cloud infrastructure we need an autonomic manager component that is deployed as a part of each allocated resource. This way this component will run at the same level of the actual offered service inside the cloud resource. 

The problem we want to solve is therefore to define a set of algorithms/heuristics to be executed by the autonomic manager, which may include a full MAPE~\cite{hornautonomic} loop (which includes Monitoring, Analysis, Planning, and the Execution of allocation/deallocations actions) to satisfy the constraints of the Service Level Agreement (SLA) contract and at the same time to reduce the costs for the amount of used resources.

For simplicity we consider a SLA contract composed of the following constraints:
\begin{itemize}
\item $R_\mathit{max}$: maximum response time for completed requests.
\item $D_\mathit{max}$: maximum percentage of incomplete requests over a given monitoring period.
\end{itemize}

Under these SLA constraints the objective is to minimize the total cost, in terms of total allocated resources $N$ over a given monitoring period, which is equivalent to keeping all the instantiated cloud resources in a given utilization range.
The benchmark used to see if the objective is correctly minimized will be to compare the measured results to the ones that would be obtained using a centralized optimal approach that has global knowledge of the system.

